On the Computational Complexity of Mechanism Design in Single-Crossing Settings

We explore the performance of polynomial-time incentive-compatible mechanisms in single-crossing domains. Single-crossing domains were extensively studied in the economics literature. Roughly speaking, a domain is single crossing if monotonicity characterizes incentive compatibility. That is, single-crossing domains are the standard mathematical formulation of domains that are informally known as ``single parameter''. In all major single-crossing domains studied so far (e.g., welfare maximization in various auctions with single-minded bidders, makespan minimization on related machines), the performance of the best polynomial-time incentive-compatible mechanisms matches the performance of the best polynomial-time non-incentive-compatible algorithms. Our two main results make progress in understanding the power of incentive-compatible polynomial-time mechanisms in single-crossing domains: We provide the first proof of a gap in the power of polynomial-time incentive-compatible mechanisms and polynomial-time non-incentive-compatible algorithms: we present an objective function in a single-crossing multi-unit auction for which there is a polynomial-time algorithm that provides an approximation ratio of $\frac{1}{2}$, yet no polynomial-time incentive-compatible mechanism provides a finite approximation (under standard computational complexity assumptions). The objective function used above is not natural. We show that to some extent this is unavoidable by providing a sweeping positive result for the most natural objective function in multi-unit auctions, that of welfare maximization. We present an incentive-compatible FPTAS mechanism for every multi-unit auction with single-crossing domains. This improves over the mechanism of Briest et al. [STOC'05] that only applies to the much simpler case of single-minded bidders.

==> acks.tex <==
We thank Liad Blumrosen for the helpful discussions. Part of the work done while the authors were affiliated with Microsoft Research.
The second and third authors are supported by ISF grant 2185/19 and BSF-NSF grant (BSF number: 2021655, NSF number: 2127781).
 The third author is supported by an Azrieli Fellowship. 

==> formalities.tex <==
\section{Formalities}\label{sec-formalities}

\subsection{
Multi-Unit Auctions}
\src{Note to Moshe -- as we discussed, maybe remove it?}
Consider a multi-unit auction setting with $m$ identical items and $n$ agents. 
{An outcome of a multi-unit auction is an allocation of the items to the agents. 
An allocation is represented by a vector} 
of quantities $(s_1,\ldots,s_n)$
such that $\sum_i s_i \le m$, where  $s_i\in [m]$ is the number of items that player $i$ gets. We denote with $\mathcal S^m$ the set of all possible allocations of $m$ items to $n$ players.  
%\sout{i.e.:}
%$$\cancel{\mathcal S^m=\{ (s_1,\ldots,s_n)\hspace{0.25em}|  \hspace{0.25em} \forall i\in[m] \hspace{0.25em} s_i\in \{0,1,\ldots,m\} \hspace{0.5em} \& \hspace{0.5em} \sum_i s_i \le m  \}}$$
% For every $\alpha \in [0,1]$,
% we say that an allocation $(S_1,\ldots,S_n)$
% $\alpha$-approximates the welfare if: $$\sum_i v_i(S_i)\ge \alpha \cdot \big[\argmax_{(A_1,\ldots,A_n)\in \mathcal S}\sum_i v_i(A_i)\big]$$ 
For multi-unit auction with $m$ items, an  \emph{$m$-item multi-unit valuation} is a function $v:[m]\to\mathbb{R}_+$ 
that assigns
a value for each quantify the agent receives. We assume that every valuation is normalized ($v(0)=0$) and monotone ($v(s+1)\geq v(s)$ for every $s\in [m-1]$). 
An \emph{$m$-item multi-unit domain} $\mathcal V^{m}$ is a set of multi-unit  valuations over $m$ items. 

A \emph{multi-unit auction with $m$ items} is defined by an $m$-item multi-unit domain for each of the agents. 
A \emph{multi-unit auction} is defined by a multi-unit auction with $m$ items, for every $m$. For a multi-unit auction, if  all $m$-item multi-unit domains are single crossing then we say that it is a \emph{multi-unit single-crossing auction}. {If all the valuations in all the multi-unit domains have only integral values, then we say that it is a \emph{multi-unit integer auction}.} Throughout the paper, we assume that all valuations only have integral values, and every multi-unit auction we consider is a multi-unit integer auction. Observe that this means that every domain we consider is countable. \src{We need to discuss representation of numbers...}

\sre{\sout{In the context of multi-unit auctions, we say that an allocation rule is \emph{quantity monotone} if for every player $i$, for every valuation profile of the other players $v_{-i}\in V_{-i}$, and for every
$\overline{v}_i\succ v_{i}\in V_i$ 
% such that $\overline{v}_i,v_{i}\in V_i$, 
it holds that 
the number of items that player $i$ receives given $(\overline{v}_i,v_{-i})$ is at least the number of items that player $i$ gets given $(v_i,v_{-i})$. Note that since we assume that valuation functions satisfy free disposal, 
% \src{\sout{any}} 
every quantity monotone rule satisfies (value) monotonicity.}}

==> payments.tex <==
\section{Payment Computation in Single-Crossing Domains}\label{sec-payment}
We now shift gears and present another set of results that deals with the hardness of computing the payments in single-crossing domains. Recall that an (ex-post) incentive-compatible mechanism must compute in every instance both the allocation and the payments. The question of whether there exists an implementable social-choice function such that the payments implementing it are much harder to compute than its allocation was posed by Fadel and Segal \cite{FS09} in a communication-complexity setting.  \cite{BBNS08} demonstrate a binary single-parameter setting for which the communication complexity of computing the allocation function is $cc(f)$ whereas the communication complexity of computing the payment is $n\cdot cc(f)$. In \cite{DR21,RSTWZ21}, the first exponential separation between computing the allocation and payment computation is achieved. In particular, in \cite{DR21} this separation is achieved even for a linear single-parameter domain. In addition, 
recall that \cite{DR21} have shown that when taking the lens of communication complexity, monotone social-choice functions in linear domains satisfy that truthful-in-expectation payment computation always comes for free, while deterministic  payment computation is sometimes %possibly 
\textquote{hard}. 
% \cite{ourpaper} have shown that if we assume that bidders are risk-neutral, then the overhead of computing 

The above hardness results are all in the communication-complexity model.  In contrast, in Appendix \ref{subsec-hardness},
we present a separation in the Turing machine model: there exists an implementable allocation function $f$ in a linear  {single-parameter} domain such that computing $f$ takes polynomial time, but computing the associated payments is $\#P-$hard. This result essentially takes the analogous result of \cite{DR21} in the communication setting, and ``adapts'' it to the Turing machine model. In Appendix \ref{subsec-expectation},
 we observe that the computational burden of truthful-in-expectation implementations is always small for single-crossing domains. Hence, there is a gap between randomized and deterministic implementations in computational complexity as well.





\subsection{A Social-Choice Function that is Easy to Compute and Hard to Incentivize} \label{subsec-hardness}
% \src{This section still needs some editing, but it is quite similar to Section \ref{sec-fptas-hard}, so I think it is best to wait until the former is finished before proofreading and writing a new version to this one.}
% \shirinote{We  need to decide whether we want this section or not.
% On one hand we already have the FPTAS payment computation hardness in section \ref{sec-fptas-hard}, but it is for the linear setting, so maybe we want to put it in the appendix? if we keep it,  then I need to change some notation here.}
In this section we show that there exists a monotone social-choice function in a linear domain (which is a special case of single-crossing domain) that is computable in polynomial time, but
every deterministic incentive-compatible mechanism that realized it is reducible to $\sharp SAT$, so it is $\sharp P$-hard.
% \mbe{turning it to deterministic incentive-compatible mechanism require solving computationally hard problems (it is $\sharp P$-hard). }
%computing an incentive-compatible mechanism for it is \textquote{hard}.
We remind that linear domains satisfy that  each player has a function $w:\mathcal{A}\to \mathbb{R}$ and a set of scalars $\Theta$ such that $V_i=\{ \theta\cdot w \hspace{0.25em} | \hspace{0.25em} \theta \in \Theta\}$.
% As a first step, we have investigated whether there exists a monotone social choice  function in a single parameter domain that can be computed efficiently, but will satisfy that computing an ex-post incentive-compatible mechanism for it is \textquote{hard}. 
 \cite{DR21} have shown that linear settings exhibit of payment computation in the communication complexity model. To replicate this gap for \emph{computational complexity}, we build on that result:
\begin{theorem}\label{sp-thm}
	There exists a social-choice function $f$
 % f:V_A\times V_B\to \mathcal [m]\times [m]$ 
 % \mbc{maybe replace  $\mathcal S$ by $[m]\times [m]$?}$
 in a multi-unit auction with  $m$ items and two players with {linear}
 %OLD
 %single-crossing 
 valuations %\mbc{the valuations are }, 
	such that: 
	\begin{enumerate}
		\item There exists an algorithm that computes $f$ in polynomial time. 
		\item  		The problem of computing any ex-post incentive-compatible implementation of 
		%OLD: An ex-post incentive-compatible implementation for
		$f$ is $\sharp P$-hard.
	\end{enumerate}
\end{theorem}
\begin{proof}
We begin by describing the domains of Alice and Bob. The domains of Alice and Bob are additive, i.e. for every number of items $s$ it holds that $w_A(s)=w_B(s)=s$.   
% OLD
%\sre{are not only linear, but also additive.}
% are very simple in the sense that they are linear
% and parameterized by their private information. 
% \sre{Alice holds a scalar $\theta_A$ such that her value for one item is $\theta_A$, her value for two items is $2\theta_A$ and so on.}
%OLD
%In other words, Alice's value for one item is her scalar $\theta_A$, for two items her value is $2\theta_A$, and so on. 
% The same holds for Bob with respect to his private information $\theta_B$. 
% The domains of both Alice and Bob are not only single crossing,  have a special linear structure: each of them has a private scalar $\theta$ such that his value for every item is $\theta$. 
% We remind that a linear domains consists of a public function and a set of scalars. 
% The set of scalars of Alice is $R_A=\{0,\frac{1}{8m^2},\frac{2}{8m^2},\ldots,m-\frac{1}{8m^2}, m\}$. 
The set of scalars of Alice is $\Theta_A=[0,m]$ and 
the set of scalars of Bob is $\Theta_B=\{0,\ldots, x-1\}$, where $x$ is the number of $3-SAT$ formulas with $\log m$ variables. 




To construct the social-choice function, we associate almost every  scalar of Alice with an assignment to $\log m$ variables: we associate all scalars in $(0,1)$ to one assignment, all scalars in   $[1,2)$ to the next assignment (according to some arbitrary order), and the same holds for the scalars in $[2,3)$ and so on and so forth. 
We denote with $a_{\theta}$ the assignment that is associated with a scalar of Alice $\theta\in \Theta_A$. Note that  $0$ and $m$ are the only scalars in $\Theta_A$ that are not associated with any assignment.  
Similarly, every scalar of Bob is associated with a $3-SAT$ formula with $\log m$ variables, such that every  valuation is matched with a  different formula. 

Now, we denote with $\phi_B$ the formula is associated with Bob's valuations, and denote an allocation of items to Alice and Bob with
$(s_A,s_B)$, where $s_A$ and $s_B$ stand for the number of items of Alice and Bob (respectively). 
% Similarly, we denote with $f_\theta$ the formula that is associated with a scalar $\theta$ of Bob.
% We denote an allocation of the items to Alice and Bob with 
% is the number of items that Alice gets and $s_F$ is the number of items of Bob.
We define the social-choice function $f$ as follows:
% \sre{With a slight abuse of notation, we write the social-choice function $f$ as a function of $\Theta_A\times \Theta_B$ instead of $V_A\times V_B$:}
% OLD
%The social-choice function $f$ is as follows:
\begin{equation*}
	f(v_A,v_B)=
	\begin{cases}
	 (\lfloor\theta_A \rfloor ,0)   &\qquad \theta_A=0 \text{ or } \theta_A=m  \\
		 (\lfloor \theta_A \rfloor + 1,0)   &\qquad 
		\text{${\lfloor \theta_A\rfloor}$ satisfies $\phi_{B}$ .} \\
		(\lfloor \theta_A \rfloor,0)
		&\qquad \text{otherwise.}
	\end{cases} 
\end{equation*} 
where $\theta_A$ is the scalar that is associated with Alice's valuation and
$\phi_B$ is the SAT formula that is associated with Bob's valuation. Note that we refer to $\lfloor \theta_A\rfloor $ both as a number and as an assignment to $\log m$ variables interchangeably. 
Throughout the proof, we slightly abuse notation by sometimes describing $f$ as a function of the valuations $v_A,v_B$ and sometimes describing it as a function of the scalars $\theta_A,\theta_B$.   
% \shirinote{TODO if time permits - a figure for the function $f$}
% We use a continuous domain to guarantee uniqueness of payments \mbc{this is only up to the normalization term} for Alice, as guaranteed by Myerson's Lemma \cite{AT01,Mye81}.  
% \mbc{I think we wnat to prove a claim for all payments, not only normalized ones. For that we need to look at the differences of payments.} 
% for Alice is necessarily identical to the payment specified in Myerson's Lemma \cite{AT01,Mye81}.
To keep the representation size logarithmic in $m$, note that for every $(\theta_A,\theta_B)\in \Theta_A\times \Theta_B$, $f(\theta_A,\theta_B)=f(\lfloor \theta_A \rfloor,\theta_B)$, so we assume that Alice writes $\lfloor \theta_A \rfloor$ on the input tape, which takes  $O(\log m)$ bits.\footnote{Another way to handle this issue is to define a discrete scalar space for Alice, but with $poly(m)$ fractions between every two subsequent integers. Then, we can show \textquote{approximate} uniqueness of payments, i.e. that a normalized payment scheme is necessarily very close to the formula provided in Myerson's Lemma, while keeping the number of bits on the input tape logarithmic in $m$.}
%OLD
% Observe that the precision of the scalar space of Alice is infinite. However, by definition for every $(\theta_A,\theta_B)\in \Theta_A\times \Theta_B$, $f(\theta_A,\theta_B)=f(\lfloor \theta_A \rfloor,\theta_B)$. Thus, $f$ can be computed given $\lfloor \theta_A \rfloor$, so we assume that Alice writes $\lfloor \theta_A \rfloor$ on the input tape, which takes  $O(\log m)$ bits. 
% To keep the representation size logarithmic in $m$, we assume that $\lfloor \theta_A \rfloor$ is written on the input tape, instead of $\theta_A$.
The scalar space of Bob can be represented with  $poly\log(m)$ bits, 
% \shirinote{TODO - to verify it. Maybe it's polylog?}, 
so an algorithm is considered  efficient if it runs in $poly\log(m)$ time. 


\begin{lemma}
$f$ is monotone and hence implementable.
\end{lemma}
\begin{proof}
$f$ is clearly monotone for Bob, because he always gets no items. 
% We denote with $f_A(v_A,v_F)$ the number of items that $f$ allocated to Alice given the valuation profile $(v_A,v_F)$.  
To prove monotonicity for Alice, fix $\theta_B\in \Theta_B$ and $\theta_A^1 \preceq \theta_A^2 \in \Theta_A$. 
Observe that: 
$$f_i(\theta_A^2,\theta_B))\ge \lfloor \theta_A^2 \rfloor \ge \lfloor \theta_A^1 \rfloor +1 \ge f_i(\theta_A^1,\theta_B))$$
which completes the proof. 
\end{proof}


\begin{lemma}
$f$ can be computed in polynomial time. 
\end{lemma}
\begin{proof}
To compute $f$, all we need to do is 
% If the input of Alice is $\lfloor \theta_A \rfloor$, we only need 
to write  $0$ on the output scalar for the allocation of Bob and decide whether Alice wins $\lfloor \theta_A \rfloor$ or $\lfloor \theta_A \rfloor+1$ items. For that, we need to check whether the assignment that $\lfloor \theta_A \rfloor$ represents satisfies the formula that $v_B$ encodes. It is easy to see that it can be done in at most $poly\log(m)$ time. 
\end{proof}
Now, it remains to show that computing an incentive-compatible mechanism that implements $f$ is $\sharp P-hard$. 
% Observe that since Bob always gets zero items, the payment scheme of $P_F\equiv 0$ incentivizes him to report his true scalar for every scalar for Alice. Computing $P_F$ is trivial.  
We prove the theorem by showing that every incentive-compatible mechanism can be used to count the number of assignments that satisfy a $3-SAT$ formula with $\log m$ variables, {thus solving $\sharp 3-SAT$, a $\sharp P-hard$ problem}:
% (Proposition \ref{prop-normalized-is-hard}). 
% Then, we proceed by showing that a mechanism that is not normalized for $f$ with running time $t$ can be used to construct a normalized mechanism for $f$ in time $\mathcal O(t)$ (Proposition \ref{prop-normalizing}). 
% Thus,  computing any incentive-compatible mechanism for $f$ reduces to $\sharp SAT$, so it is $\sharp P-hard$.  
% reduces to  computing every payment scheme $p_A$ of Alice that implements the social-choice function $f$ is $\sharp P-hard$. We do it in two steps.
% First, we prove that computing a normalized payment scheme for Alice is $\sharp P-hard$ (Proposition \ref{prop-normalized-is-hard}). Then, we proceed by showing that by making two calls to a payment scheme that is not normalized, we can design a normalized payment scheme for her (Proposition \ref{prop-normalizing}). 
% The two propositions jointly imply that counting
% the number of assignments that satisfy a SAT formula reduces to incentive-compatible mechanism for the social-choice function $f$. Let
\begin{proposition}\label{prop-normalized-is-hard}
Let $\mathcal M=(f,P_A,P_B)$ be an incentive-compatible mechanism.
% Let $M$ be a normalized incentive-compatible mechanism for the social-choice function $f$, such that the payment scheme of Alice is $p_A^{norm}:\Theta_A\times \Theta_B\to \mathbb{R}$. 
Let $\phi$ be a formula that has $\ell$ assignments that satisfy it. Denote with $\theta_B$ the scalar of Bob that is associated with the formula $\phi$.
\emph{Then}:
$$
P_A(m,\theta_B)-P_A(0,\theta_B)= \frac{m^2+m}{2} -\ell 
$$
% Let $\phi$ be a formula that has $\ell$ assignments that satisfy it, and let $\phi'$ be a formula that has $\ell'$ assignments that satisfy it. 
% Denote with $\theta_B,\theta_B'$ the scalars of Bob that are associated with the formulas $\phi,\phi'$ respectively. Then, if $\ell \neq \ell'$, it implies that 
% $ p_A(m,v_\phi) \neq  p_A(m,v_\phi')$.
\end{proposition}
% \begin{proposition}\label{prop-normalized-is-hard}
% Let $p_A$  be the payment scheme of Alice in an ex-post incentive-compatible normalized mechanism that implements the function $f$. 
% Let $\phi$ be a formula that has $\ell$ assignments that satisfy it, and let $\phi'$ be a formula that has $\ell'$ assignments that satisfy it. 
% Denote with $\theta_B,\theta_B'$ the scalars of Bob that are associated with the formulas $\phi,\phi'$ respectively. Then, if $\ell \neq \ell'$, it implies that 
% $ p_A(m,v_\phi) \neq  p_A(m,v_\phi')$.
% \end{proposition}

\begin{proof}
By Myerson's Lemma \cite{AT01,Mye81}, we have that every payment scheme for Alice satisfies that: 
$$
P_A(\theta_A,\theta_B)-P_A(0,\theta_B)=\theta_A\cdot f_A(\theta_A,\theta_B)- \int_0^{\theta_A}f_A(z,\theta_B)dz   
$$
where $f_A(\theta_A,\theta_B)$ is the number of items that Alice wins given the instance $(\theta_A,\theta_B)$.
Observe that by the construction of the function $f$ and by Myerson's Lemma, we have that:
\begin{align*}
    P_A(m,\theta_B)&= m^2 - \int_0^{m}f_A(z,\theta_B)dz \\
    &= m^2 
    	-\sum_{\mathclap{\substack{i=0 \\ \text{the assignment}
    	\\ \text{associated with}
    	\\ \text{$\theta_A=i$ does not}
    	\\ \text{satisfy $\phi$}}}}^{m-1} i 
    	\hspace{2.5em}
    	- \sum_{\mathclap{\substack{i=0 \\ \text{the assignment}
    	\\ \text{associated with}
    	\\ \text{$\theta_A=i$}
    	\\ \text{satisfies $\phi$}}}}^{m-1} (i+1)\\
    	&= m^2 - \sum_{i=0}^{m-1}i -\ell \\
    	&= \frac{m^2+m}{2}-\ell 
\end{align*}
which completes the proof. 
% Let $\tilde{f}$ be another social-choice function, which is identical to $f$ except that it is defined for the case where the scalar space of Alice is an interval, whereas $f$ is defined on a discrete scalar space of Alice. 
% The domain of Alice, $\tilde{\Theta}_A$, is $[0,m]$ and the domain of Bob remains the same: $\tilde{\Theta}_F=\Theta_B$. For every $(\tilde{\theta}_A,\tilde{\theta}_F)\in \tilde{\Theta}_A\times \tilde{\Theta}_F$, $\tilde{f}(\tilde{\theta}_A,\tilde{\theta}_F)=f(\lfloor \tilde{\theta}_A \rfloor,\tilde{\theta}_F)$. Now, observe that by Myerson Lemma , we have that:
\end{proof}
\end{proof}

\subsection{Computation of Truthful-in-Expectation Payments} \label{subsec-expectation}
% \src{TODO - make sure the payment formula here is identical to the preliminaries}
% \mbc{This result is not really a Theorem and is not really ours, it is well known. Consider making it an observation, moving this section to the appendix, and only pointing to it when saying that deterministic payment computation is hard, as an observation that completes the picture.}
Recall that \cite{DR21} have shown that when taking the lens of communication complexity, monotone social-choice functions in linear domains satisfy that truthful-in-expectation payment computation always comes for free, while deterministic  payment computation is sometimes %possibly 
\textquote{hard}. We now observe that this is the case also for single-crossing domains in the computational-complexity model. 

For that, we remind that a randomized mechanism $\mathcal M=(f,P_1,\ldots,P_n):V_1\times\cdots\times V_n\to \mathcal A \times \mathbb{R}^n$  is \emph{truthful in expectation} if for every player $i$, for every $v_i,v_i'\in V_i$, and for every $v_{-i}\in V_{-i}$: 
$$
\E [v_i(f(v_i,v_{-i}))
-P_i(v_i,v_{-i})] \ge
\E [v_i(f(v_i',v_{-i}))
-P_i(v_i',v_{-i})]
$$
where the expectation is taken over the random coins of the mechanism. 
Similarly to Sections \ref{sec-alg-k} and \ref{sec-alg}, we assume we have access to extended value queries and that the input is given as $(t_1,\ldots,t_n)$, where $t_i$ is the index of the $t_i$'th valuation in the domain of player $i$ {($v_i=v_i^{[t_i]}$)}. 
% \shirinote{I think that we have to use the term \textquote{truthful} here if we want to talk about \textquote{truthful in expectation} mechanisms. Unless \textquote{incentive-compatible in expectation} makes any sense.} 
%OLD: 
%In this section, we show that if we consider computational complexity - then this gap between randomized and deterministic  persists, not only for the linear domain but also for domains that satisfy the single-crossing property. The social-choice function where deterministic payment computation is \textquote{hard} can be found in Section \ref{sec-fptas-hard}, whilst in this section we  show that the computational burden of truthful in expectation implementations is always small for multi-unit single-crossing domains. 
% For that, we remind that an unbiased estimator for the Myerson payment formula for linear domains can be obtained by sampling the 
% value of the function
% %OLD (wrong):height of the integral 
% at a random point (see \cite{archer-papadimitriou-talwar-tardos,bks-implicit}). We use the same technique to obtain 
% \mbc{remove this: ? } \src{remove what? I don't think that I understand you..} The same technique can also be used 
% to obtain 
%  an unbiased estimator for
% the payment formula of countable multi-unit single-crossing domains.  
% We now show that by \textquote{discretizing} this technique, 
% we can obtain an unbiased estimator for the payment formula of multi-unit single-crossing domains.  \mbc{this is unclear} 
% \src{I currently write the algorithm for multi-unit auctions, because it requires order over the alternatives. I'll write it for multi-unit auctions for now and I think that if we use the right single crossing definition, then we can easily generalize it to more settings.}
% \src{See if I can adapt this for domains of countable size. Also --  this can also work for continuous domains.}
{We next observe that generating a random variable for the payment that has  the right expectation is straightforward: The proof of the next claim is a straightforward adaption of the well known trick \cite{archer-papadimitriou-talwar-tardos,bks-implicit} of obtaining an unbiased estimator for the Myerson payment formula by sampling the value of the function at a random point.}
\begin{claim}
Let $f:V_1\times\cdots\times V_n\to \mathcal A$ be a monotone deterministic social-choice function in {a single-crossing setting}. {Then,
a truthful-in-expectation mechanism\footnote{That is ex-post IR.} for $f$ can be computed by executing its algorithm $n$ additional times, and making $3n$ extended value queries (in addition to the time and queries needed for the computation of $f$).} 
% a multi-unit  auction
% such that for every player $i$ the domain $V_i$ is a \mbe{finite} % we take the log of the size
% single-crossing domain. 
% {If $f$ can be computed in time $T$ with $q$ domain queries, then}
% \emph{Then}, every such social-choice function $f$ that can be computed in time $T$ \mbc{change to $T$ throughout?} with $q$ queries has
% there exists a truthful-in-expectation mechanism that implements it in time $poly(n,T)$ and with 
%$n$ additional
% $poly(n,q)$ extended value queries. 
% \mbc{there is another standard trick one can use - instead of running the sampling for each agent, one can pick a random agent and charge him $n$ times the prior payment. This gives the same result but with lower complexity. Thus,  we can generate the right expected payment using just one additional execution of the allocation rule (on a randomly picked input). Actually, maybe better to present it like that.} 
\end{claim}
% In particular, it implies that if the domains are of size  $poly(m)$, then a truthful-in-expectation mechanism has only $poly\log (m)$ computational overhead. 
\begin{proof}
Let $(v_1,\ldots,v_n)$ be a valuation profile. 
Fix a player $i$. 
By Proposition \ref{prop-mono-iff-sc}, by some algebraic manipulations it can be shown that the following payment  \emph{deterministically} implements $f$ (since all the summands that do not cancel out are equal to the summands in Proposition \ref{prop-mono-iff-sc}):
\begin{equation} \label{eq-myerson-payment2}
    P_i(v_i^{[t_i]},v_{-i})= v_i^{[l]}(f_i(v_i^{[t_i]},v_{-i}))-\sum_{d=1}^{t_i} \big[v_i^{[d]}(f_i(v_i^{[d-1]},v_{-i}))- v_i^{[d-1]}(f_i(v_i^{[d-1]},v_{-i})) \big]
    \end{equation}
where we remind that $v_i^{[0]},\ldots,v_i^{[t_i]}$ are the first $t_i+1$ valuations according to total order $\succ_i^{v}$ of the domain $V_i$. 
Hence, to compute a truthful-in-expectation mechanism, it suffices that the payment of player $i$ will be a random variable 
% payment that is truthful-in-expectation, it suffices to compute a random variable 
that is equal in expectation to (\ref{eq-myerson-payment2}). For that, our truthful-in-expectation mechanism outputs the following payment for player $i$:
$$
\hat{P}_i = v_i^{[t_i]}(f_i(v_i^{[t_i]},v_{-i})) - t_i \cdot \big(v_i^{[d+1]}(f_i(v_i^{[d]},v_{-i}))- v_i^{[d]}(f_i(v_i^{[d]},v_{-i})) \big)
$$
where $d$ is an index that we sample uniformly from $\{1,\ldots,t_i\}$. 
Now, observe that:
\begin{align*}
    \E_{d}[\hat{P}_i] &=
    v_i^{[l]}(f_i(v_i^{[l]},v_{-i})) - t_i \cdot  \E_d[v_i^{[d]}(f_i(v_i^{[d-1]},v_{-i}))- v_i^{[d-1]}(f_i(v_i^{[d-1]},v_{-i}))]  \\
    % &\text{(linearity of expectation)} \\
    &= v_i^{[t_i]}(f_i(v_i^{[t_i]},v_{-i})) - t_i \cdot 
    \sum_{d=1}^{t_i}\frac{1}{t_i}\Big[    v_i^{[d]}(f_i(v_i^{[d-1]},v_{-i}))- v_i^{[d-1]}(f_i(v_i^{[d-1]},v_{-i}))\Big] \\
    % &\text{(law of the unconscious statistician)} \\
&=v_i^{[t_i]}(f_i(v_i^{[t_i]},v_{-i}))-\sum_{d=1}^{t_i} \big[v_i^{[d]}(f_i(v_i^{[d-1]},v_{-i}))- v_i^{[d-1]}(f_i(v_i^{[d-1]},v_{-i})) \big]
\end{align*}
where the second equality is due to the law of the unconscious statistician.
%\mbc{the parenthesis in the second line should be after the $1/l$ term, changed}
Hence, $\hat{P}_i$ is indeed an unbiased estimator for (\ref{eq-myerson-payment2}).

Note that computing $\hat{P}_i$ requires  simulating the algorithm for $f$ to get the alternative  $a=f(v_i^{[d-1]},v_{-i})$ 
and then making two extended value queries to obtain $v_i^{[d]}(a)$ and $v_i^{[d+1]}(a)$, so the time and query complexity are as in the statement.    
\end{proof}

==> single-crossing-prop.tex <==
\section{Monotonicity and Incentive Compatibility in Discrete Single Crossing Settings - Proof of Proposition \ref{prop-mono-iff-tru}}
\label{sec-hermalin-proof} 
\shirinote{the proof, if used eventually, should be slightly changed because of a slight modification in the payment formula}
For the first direction, assume that $f$ has payment schemes $P_1,\ldots,P_n$ such that  the direct mechanism $\mathcal M=(f,P_1,\ldots,P_n)$ is incentive compatible. To prove that $f$ is monotone, fix a player $i$, two valuations $v_i^k \prec v_i^l \in V_i$  and a valuation profile $v_{-i}\in V_{-i}$ of the other players. Denote $f(v_i^k,v_{-i})$ with $a_k$ and
$f(v_i^l,v_{-i})$ with $a_l$.
We want to prove that:
$$
v_i^k(a_l) \ge  v_i^k(a_k) 
$$
Since $\mathcal M$ is incentive compatible: 
\begin{equation}\label{eq-mono-1}
    \begin{multlined}
        v_i^k(a_k)
-P_i(v_i^k,v_{-i}) \ge
v_i^k(a_l)
-P_i(v_i^l,v_{-i}) \implies
\\ P_i(v_i^l,v_{-i}) -P_i(v_i^k,v_{-i}) \ge v_i^k(a_l) - v_i^k(a_k)
    \end{multlined}
\end{equation}
And similarly:
\begin{equation}\label{eq-mono-2}
    \begin{multlined}
        v_i^l(a_l)
-P_i(v_i^l,v_{-i}) \ge
v_i^l(a_k)
-P_i(v_i^k,v_{-i}) \implies
\\ 
v_i^l(a_l) - v_i^l(a_k) \ge P_i(v_i^l,v_{-i}) -P_i(v_i^k,v_{-i})
    \end{multlined}
\end{equation}
By (\ref{eq-mono-1}) and (\ref{eq-mono-2}):
\begin{equation}\label{eq-conclus}
v_i^l(a_l) - v_i^l(a_k) \ge 
v_i^k(a_l) - v_i^k(a_k)    
\end{equation}
Now, assume towards a contradiction that $v_i^k(a_l)<v_i^k(a_k)$. In this case, $v_i^k(a_k)-v_i^k(a_l)>0$, so the single-crossing condition implies that $v_i^l(a_k)-v_i^l(a_l)>v_i^k(a_k)-v_i^k(a_l)$, which is a contradiction to (\ref{eq-conclus}). 
% Note that it implies that $v_i^k(f(v_i^l,v_{-i})) \ge  v_i^k(f(v_i^k,v_{-i}))$. The reason for it is that if $v_i^k(f(v_i^l,v_{-i})) <  v_i^k(f(v_i^k,v_{-i}))$, it would have meant that $v_i^l(f(v_i^l,v_{-i})) - v_i^l(f(v_i^k,v_{-i})) \le 
% v_i^k(f(v_i^l,v_{-i})) - v_i^k(f(v_i^k,v_{-i}))$. 
% So by definition, $f_i(v_i^l,v_{-i}) \succeq_i f_i(v_i^k,v_{-i})$.


For the other direction, assume that $f$ is monotone. Fix again a player $i$, two valuations $v_i^k \prec v_i^l \in V_i$  and a valuation profile $v_{-i}\in V_{-i}$ of the other players. We want to prove that the two following assertions hold:
\begin{enumerate}
    \item 
    $v_i^k(f(v_i^k,v_{-i}))
-P_i(v_i^k,v_{-i}) \ge
v_i^k(f(v_i^l,v_{-i}))
-P_i(v_i^l,v_{-i})$. \label{item-part1}
\item $v_i^l(f(v_i^l,v_{-i}))
-P_i(v_i^l,v_{-i}) \ge
v_i^l(f(v_i^k,v_{-i}))
-P_i(v_i^k,v_{-i})$. \label{item-part2}
\end{enumerate}
where $P_i$ is the payment that is specified in equation (\ref{eq-myerson-payment}). For the former part, observe that:
\begin{gather*}
v_i^k(f(v_i^k,v_{-i}))
-P_i(v_i^k,v_{-i})= \sum_{d=0}^{k-1} \big[ v_i^{d+1}(f(v_i^d,v_{-i})) - v_i^{d}(f(v_i^d,v_{-i})) \big] \\
v_i^k(f(v_i^l,v_{-i}))
-P_i(v_i^l,v_{-i})= 
v_i^k(f(v_i^l,v_{-i}))-
v_i^l(f(v_i^l,v_{-i}))+\sum_{d=0}^{l-1} \big[v_i^{d+1}(f(v_i^d,v_{-i}))- v_i^{d}(f(v_i^d,v_{-i})) \big]
\end{gather*}
Therefore:
\begin{equation}\label{eq-iff}
\begin{aligned} v_i^k(f(v_i^k,v_{-i}))
-P_i(v_i^k,v_{-i}) &\ge  v_i^k(f(v_i^l,v_{-i}))
-P_i(v_i^l,v_{-i}) \iff \\
\sum_{d=0}^{k-1} \big[ v_i^{d+1}(f(v_i^d,v_{-i})) - v_i^{d}(f(v_i^d,v_{-i})) \big] &\ge 
v_i^k(f(v_i^l,v_{-i}))-
v_i^l(f(v_i^l,v_{-i}))  +\sum_{d=0}^{l-1} \big[v_i^{d+1}(f(v_i^d,v_{-i}))- v_i^{d}(f(v_i^d,v_{-i})) \big] \\ \iff 
v_i^l(f(v_i^l,v_{-i})) - v_i^k(f(v_i^l,v_{-i})) &\ge 
\sum_{d=k}^{l-1} \big[ v_i^{d+1}(f(v_i^d,v_{-i})) - v_i^{d}(f_i(v_i^d,v_{-i})) \big]
\end{aligned}
\end{equation}
We remind that $f$ is monotone, so by definition for every valuation index $d$ that is smaller than $l$, we have that $v_i^d(f(v_i^l,v_{-i}))\ge v_i^d(f(v_i^d,v_{-i}))$. Since $V_i$ is a single crossing domain, it implies that:
\begin{gather*}
v_i^{d+1}(f(v_i^l,v_{-i}))- v_i^{d+1}(f(v_i^d,v_{-i}))
\ge v_i^d(f(v_i^l,v_{-i}))- v_i^d(f(v_i^d,v_{-i})) \\ \implies   
v_i^{d+1}(f(v_i^l,v_{-i}))-v_i^d(f(v_i^l,v_{-i})) \ge v_i^{d+1}(f(v_i^d,v_{-i}))-v_i^d(f(v_i^d,v_{-i})) 
\end{gather*}
Therefore:
\begin{align*}
    \sum_{d=k}^{l-1} \big[ v_i^{d+1}(f_i(v_i^d,v_{-i})) - v_i^{d}(f_i(v_i^d,v_{-i})) \big] &\le  \sum_{d=k}^{l-1} \big[ v_i^{d+1}(f_i(v_i^l,v_{-i})) - v_i^{d}(f_i(v_i^l,v_{-i})) \big] 
    % &\text{(by (\ref{eq-single-crossing}))} 
    \\
    &= v_i^{l}(f_i(v_i^l,v_{-i})) - v_i^{k}(f_i(v_i^l,v_{-i})) 
\end{align*}
which completes the proof of part \ref{item-part1}, according to the logical equivalences in (\ref{eq-iff}). 
For part \ref{item-part2}, observe that:
\begin{align}       v_i^l(f(v_i^l,v_{-i}))
-P_i(v_i^l,v_{-i}) &\ge
v_i^l(f(v_i^k,v_{-i}))
-P_i(v_i^k,v_{-i}) \iff \nonumber\\
\sum_{d=0}^{l-1} \big[ v_i^{d+1}(f(v_i^d,v_{-i})) - v_i^{d}(f(v_i^d,v_{-i})) \big] &\ge 
v_i^l(f(v_i^k,v_{-i}))-
v_i^k(f(v_i^k,v_{-i})) \nonumber \\ &+\sum_{d=0}^{k-1} \big[v_i^{d+1}(f(v_i^d,v_{-i}))- v_i^{d}(f(v_i^d,v_{-i})) \big] \iff \nonumber \\ 
\sum_{d=k}^{l-1} \big[v_i^{d+1}(f(v_i^d,v_{-i}))- v_i^{d}(f(v_i^d,v_{-i})) \big] &\ge
v_i^l(f(v_i^k,v_{-i}))-
v_i^k(f(v_i^k,v_{-i}))
\label{eq-sec-direction}
\end{align}
Now, due to the same reasons as in part \ref{item-part1}, we have that for every valuation index $d$ that is larger than $k$:
$$
v_i^{d+1}(f(v_i^d,v_{-i}))-v_i^d(f(v_i^d,v_{-i}))\ge 
v_i^{d+1}(f(v_i^k,v_{-i}))-v_i^d(f(v_i^k,v_{-i}))
$$
And therefore:
\begin{align*}    \sum_{d=k}^{l-1} \big[v_i^{d+1}(f_i(v_i^d,v_{-i}))- v_i^{d}(f_i(v_i^d,v_{-i})) \big] &\ge 
   \sum_{d=k}^{l-1} \big[v_i^{d+1}(f_i(v_i^k,v_{-i}))- v_i^{d}(f_i(v_i^k,v_{-i})) \big] \\
    &= v_i^{l}(f_i(v_i^k,v_{-i}))- v_i^{k}(f_i(v_i^k,v_{-i}))
\end{align*}
so (\ref{eq-sec-direction}) holds, and by that we complete the proof.


==> welfare-max-np-hard.tex <==
\section{Welfare Maximization is Hard For Two Single Crossing Players}
\label{sec-2-player-hard}
\sout{\sre{It is well known that exact welfare maximization is hard for known single-minded bidders in multi-unit auctions when the number of agents is large.}}
\src{It is stated as fact in Mualem Nisan, I need to find the right citation for it, but under the weird assumption that the auctioneer can "verify" the quantity so the domains are actually unknown single-minded and the reduction to knapsack still works. So I think we should delete this phrase for now.}
\shirinote{} 
However, if the number of bidders is constant, then we can find the optimal allocation efficiently (by iterating over all subsets of players, and outputting a feasible allocation with the highest welfare). 
In this section, we show that for single-crossing domains  exact welfare maximization can be computationally hard even when the number of players is small. 
% Note that for single-minded bidders, computing the optimal allocation is trivial if the number of bidders is constant: we can brute force over all possible allocations efficiently. We will use this hardness result as a basis to show that there exists an objective function that cannot be computed by  
% \begin{theorem}
% There exist a multi-unit auction with two single-crossing bidders whose valuations can be succinctly represented, such that no deterministic polynomial-time algorithm outputs the welfare-maximizing allocation, unless $P=NP$.
% \shirinote{The phrasing of this theorem is an adaptation of Theorem 2.1 in \url{https://drive.google.com/file/d/1LE9Q8TRvwFuYoyxtweCPWh7LLfqByOsy/view}.}

% MB NEW:
The \emph{welfare-maximization problem for single-crossing multi-unit domains} is the problem of finding, for every vector of valuations each from a single-crossing multi-unit domain, an allocation that maximizes the social welfare. 
\begin{theorem}
\label{thm-2-player-hard}
The welfare-maximization problem for  single-crossing multi-unit auction
is NP-hard, even with two agents.   
\end{theorem}

%There is two classes $C_A,C_F$ of single crossing multi unit domains such that every valuation is succinctly represented, and if there exists a deterministic polynomial-time algorithm that for any input outputs a welfare-maximizing allocation, then NP=P. 
The proof is an adaptation of the lower bound in \cite{dobvon12} for general valuations to single crossing domains. 
\begin{proof}
To prove the claim we
reduce $3-SAT$ to the welfare-maximization problem for single-crossing multi-unit auction with two agents. 
For that, we map the set $\Phi^k$ of 3-SAT formulas over $k$ variables %, \magenta{which we denote with $\Phi^k$,} 
to a 2-agent single-crossing multi-unit auction  over $m=2^k$ items with %two agents and
valuations that can be represented with $poly(k)= poly\log(m)$ bits.

To define the domains of valuations in this auction, we associate every $3-SAT$ formula $\phi$ with $k$ variables, %and $N= {\binom{2k}{3}} \leq 2k^3$ clauses 
with an ordinal number $x_\phi$ in 
$\mathcal X= \{1,\ldots,2^N\}$ for $N= {\binom{2k}{3}} \leq 2k^3$. Such an association from a $3$-SAT formula $\phi$ to its ordinal number $x_\phi$ can be obtained by
writing for each of the clauses, in lexicographic order, a bit that specifies whether this clauses appears in the SAT formula or not.
% We denote the ordinal number of a $3-SAT$ formula $\phi$ with $x_{\phi}$.
Thus,
we can compute
the ordinal number of each formula in $poly(k)$ time.
% We define \mbc{we never define this explicitly. maybe we should?} the ordinal numbers in a way that guarantees that the ordinal number of each formula can be computed efficiently given the formula and can be represented with $\mathcal O(\log m)$ bits.


We name the two players Alice and Bob, and name their domains with $V_A^k$ and $V_B^k$ respectively, {where each domain contains multi-unit valuations over $m=2^k$ items}.
We associate every 3-SAT formula $\phi\in \Phi^k$ with a valuation of Alice and with a valuation of Bob. 
We denote the domain of Alice by $V_A^k=\{v_{A}^\phi\hspace{0.25em}|\hspace{0.25em}
\phi\in \Phi^k\}$.
%\magenta{In fact,}   each valuation of Alice is parameterized by a formula, i.e.,  $V_A^k=\{v_{A}^\phi\hspace{0.25em}|\hspace{0.25em}\phi\in \Phi^k\}$. 
The valuation $v_A^\phi$ that is associated with the formula $\phi$ is defined as follows:
\begin{gather*}
v_A^\phi(0)=0 \\
\forall s\in \{1,\ldots,2^k\} \quad
v_A^\phi(s)=4sx_{\phi}+\phi(s)    
\end{gather*}
where we refer to every quantity  $s\in\{1,\ldots,2^k\}$ both as an integer (the value $s$) and as an assignment to $k$ binary variables.\footnote{Note that the  quantity of zero items represents no assignment. The reason for  isf
that if it would have been associated with some assignment, then $v^\phi(0)$ would have been equal to $1$  
whenever that assignment satisfies $\phi$, so  $v^\phi$ would not have been  normalized. 
}
In words, if $\phi$ is not satisfiable then $v^\phi(s)=4sx_\phi$ for every quantity $s$. If the assignment $s$ satisfies $\phi$, then $v^\phi(s)=4sx_\phi+1$. 
% For illustration, observe the valuation $v$ that is associated with the formula $\phi_1$. 
% Observe the following example for illustration. Let $\phi_1$ be the formula such that its ordinal number $x_{\phi_1}$ is equal to $1$.  Then, if $\phi_1$ is not satisfiable,  then the value for every number of items $s$ is $4s$. However,
% if the assignment $s$ satisfies the formula $\phi$, then the value for $s$ items is $4s+1$. 
\darkgreen{Note that this domain satisfies strict increasing differences, when the order of the valuations is according to the ordinal number of their SAT formulae: The reason for it is that if the {ordinal number of 
formula $\phi$ associated with a valuation $v^\phi$ is $x_\phi$,} then all its margins are necessarily equal to one of  {$\{4x_\phi-1,4x_\phi,4x_\phi+1\}$}.
{The claim holds as for any integer $x$ it holds that $4x+1< 4(x+1)-1$.}
}


% If  is satisfied by an assignment $s$, then 
% has assignments that satisfy it, then the added value of $v_A^{\phi_1}$ is $3$ for quantities that  correspond to satisfying assignments, and $2$ otherwise. 

Next, we define the domain $V_B^k$ of Bob.
Similar to Alice, the domain $V_B^k=\{v_{F}^\phi\hspace{0.25em}|\phi\in \Phi^k\}$ of Bob associates a valuation $v_B^\phi\in V_B^k$ with each formula $\phi\in \Phi^k$. The valuation $v_B^\phi$ is defined as follows:
$$
\forall s\in \{0,1,\ldots,2^k\} \quad
v_B^\phi(s)=4sx_{\phi}
$$
I.e., all his valuations are additive and  thus \darkgreen{$V_B$ is clearly a single crossing domain.}  
In addition, note that both valuations 
 of both Alice and Bob can be encoded succinctly by writing their corresponding $3$-SAT formulae using $poly(k)$ bits,
 since writing each clause requires $\mathcal{O}(\log k)$ bits,  
 and there are $poly(k)$ clauses.
 Finally, observe that for every $\phi$ and $s\in\{0,\ldots,m\}$, both $v^\phi_A(s)$ and $v^\phi_F(s)$ can be computed efficiently.

 
 
Now, the reduction is as follows.  Let $\phi\in \Phi^k$ be a $3-SAT$ formula, and let 
 $func:V_A\times V_B\to \mathcal S^m$ be a computationally efficient function that outputs a welfare-maximizing allocation, {where we remind that $m=2^k$}. 
Let $v_A^\phi$ and $v_B^\phi$ (respectively) be the valuations of Alice and Bob that correspond to $\phi$, and let $(s_A,s_F)$ be the allocation of $func$ on the input $(v_A^\phi,v_B^\phi)$.
 %OLD
 % Given a $3-SAT$ formula $\phi$, let $v_A^\phi$ and $v_B^\phi$ (respectively) be the valuations of Alice and Bob that correspond it. 

Now, observe that $\phi$ is satisfiable if and only if 
$v_A^\phi(s_A)+v_B^\phi(s_F)$ is equal to $4mx_\phi+1$, where $x_\phi$ is the ordinal number of the formula $\phi$. The reason for it is as follows. If $\phi$ is not satisfiable, then every partition of the items yields welfare of $4mx_\phi$. In contrast, if the assignment that corresponds to the quantity $s$ satisfies $\phi$, then $v_A^\phi(s)+v_B^\phi(m-s)=4mx_\phi+1$.

Also, the reduction takes polynomial time because 
\sre{the value of $v_A^\phi$ and $v_B^\phi$ of every quantity $s$ can be computed in polynomial time.}
%OLD
% \mbe{%the representation of 
% each valuation $v_A^\phi$ and $v_B^\phi$ can be computed in time $poly(k)$ given the corresponding  $3$-SAT formula that is represented using $poly(k)$ bits}.
Thus, if we can efficiently solve the welfare maximization problem we can efficiently decide for every $3-SAT$ formula if it is satisfiable or not.
\end{proof}
% \begin{remark}
% Observe that the proof of Theorem \ref{thm-2-player-hard} implies that not only the allocation problem of NP-hard, but also the decision problem (which asks whether the optimal welfare is above $x$).  
% \end{remark}


